ASSR-NeRF: Arbitrary-Scale Super-Resolution on Voxel Grid for High-Quality Radiance Fields Reconstruction

NeRF-based methods reconstruct 3D scenes by building a radiance field with implicit or explicit representations. While NeRF-based methods can perform novel view synthesis (NVS) at arbitrary scale, the performance in high-resolution novel view synthesis (HRNVS) with low-resolution (LR) optimization often results in oversmoothing. On the other hand, single-image super-resolution (SR) aims to enhance LR images to HR counterparts but lacks multi-view consistency. To address these challenges, we propose Arbitrary-Scale Super-Resolution NeRF (ASSR-NeRF), a novel framework for super-resolution novel view synthesis (SRNVS). We propose an attention-based VoxelGridSR model to directly perform 3D super-resolution (SR) on the optimized volume. Our model is trained on diverse scenes to ensure generalizability. For unseen scenes trained with LR views, we then can directly apply our VoxelGridSR to further refine the volume and achieve multi-view consistent SR. We demonstrate quantitative and qualitatively that the proposed method achieves significant performance in SRNVS.

==> figure/ablation.tex <==
\begin{figure}[t]
	\centering
	\includegraphics[width=1\columnwidth]{figure/ablation.png}
 % \vspace{-5mm}
    \caption{ 
        Ablation study of applying VoxelGridSR to volumetric representations with a cross-scene RGBNet (left) and with a per-scene RGBNet (right). 
    }
    \vspace{-3mm}
	\label{fig:ablation}
\end{figure}

==> table/sr_compare.tex <==
\begin{table*}[hbt!]
	\centering
 \resizebox{\textwidth}{!}{%
	\begin{tabular}{|c||c c c| c c c|}
		\hline
    \ &\multicolumn{3}{|c}{x2}
        &\multicolumn{3}{|c|}{x4}\\
		\cline{2-7}
		 dataset: LLFF ~\cite{mildenhall2019local} &  PSNR $\uparrow$ & SSIM $\uparrow$  & LPIPS $\downarrow$ & PSNR $\uparrow$ & SSIM $\uparrow$  & LPIPS $\downarrow$  \\
		\hline\hline
  %           TensoRF \cite{chen2022tensorf} & 24.65 & 0.771 & 0.268 & 22.78 & 0.658 & 0.417 & \textbf{22.29} & \textbf{0.632} & 0.467 & \textbf{22.29} & \textbf{0.656} & \textbf{0.489}\\
		% \hline
  %           Instant-ngp \cite{M_ller_2022} & \textbf{0.909} & \textbf{0.906} & 0.860 & 0.875 & 0.840 & 0.841 & dsf & adf & 0.840 & 0.841 & dsf & adf\\
		% \hline
            TensoRF \cite{chen2022tensorf}+ Real-ESRGAN \cite{wang2021realesrgan} & 24.44 & 0.782 & 0.249 &  23.49 & 0.721 & \textbf{0.353} \\
		\hline
            TensoRF \cite{chen2022tensorf}+ SwinIR \cite{Liang2021SwinIRIR} & 25.40 & 0.811 & 0.258  & 24.35 & 0.741 & 0.417 \\
		\hline\hline
            ASSR-NeRF (ours)  & \textbf{26.09} & \textbf{0.827} & \textbf{0.220} & \textbf{25.03} & \textbf{0.769} & 0.376 \\
		\hline
		
	\end{tabular}
}

\caption{Comparisons with 2D image SR methods on LLFF~\cite{mildenhall2019local}: ASSR-NeRF directly renders HR novel views. For comparison, TensorRF~\cite{chen2022tensorf} first renders LR novel views, then SOTA image SR methods super-resolve the views to HR. Our approach achieves the best performances in all the metrics.}
	\label{tab:nerfsr}
\end{table*}
